Interleaved Weighted Round-Robin: A Network Calculus Analysis

Weighted Round-Robin (WRR) is often used, due to its simplicity, for scheduling packets or tasks. With WRR, a number of packets equal to the weight allocated to a flow can be served consecutively, which leads to a bursty service. Interleaved Weighted Round-Robin (IWRR) is a variant that mitigates this effect. We are interested in finding bounds on worst-case delay obtained with IWRR. To this end, we use a network calculus approach and find a strict service curve for IWRR. The result is obtained using the pseudo-inverse of a function. We show that the strict service curve is the best obtainable one, and that delay bounds derived from it are tight (i.e., worst-case) for flows of packets of constant size. Furthermore, the IWRR strict service curve dominates the strict service curve for WRR that was previously published. We provide some numerical examples to illustrate the reduction in worst-case delays caused by IWRR compared to WRR.

==> Proofs.tex <==

%%%%%%%%%%%%%%%%          Main Results    %%%%%%%%%%%%%
\section{Main Results} \label{sec:Results}

\subsection{Strict Service Curves}
%% %%%%%%%%%%%%The Strict Service Curve Theorem of Interleavd WRR%%%%%%%%%%%% 
\begin{theorem}[Strict Service Curve of Interleaved WRR]
Let $S$ be a server, offering a strict service of super-additive curve $\beta$, shared by $n$
flows $R_1,...,R_n$. Each flow $f$ has a minimum packet size $l^{min}_f$ and a maximum packet size $l^{max}_f$ 
and a weight $w_f$. Then, $S$ offers to each flow $R_f$ a strict
residual service curves:
\begin{equation}
\beta_f \left( t \right) = \left( \lambda_1 \otimes U_f \right) \left( \beta \left( t \right) \right)
\end{equation}	
Where $U_f$ is defined as described below:
\begin{center}
$U_f(x) = \sum_{k=0}^{w_f - 1}\left( \nu_{l^{min}_f,L_{tot}} \otimes \delta_{\psi_f(kl^{min}_f))} \right) (x)$
\end{center}
Where $\nu_{h,T}$ is the stair function and $\lambda_r$ is a guaranteed rate $r$ \cite{le_boudec_network_2001}, with $Q_f =  \sum_{g,g \neq f} w_gl^{max}_g$, $q_f = w_fl^{min}_f$, and $L_{tot} =q_f + Q_f$. Let define $\phi_{f,g}: x \mapsto \lfloor \frac{x}{w_f} \rfloor w_g  +  \left[w_g - w_f\right]^+ + min(x \mod w_f+ 1 ,  w_g)$. Then, $\psi_f$ is defined as below:
\begin{center}
$\psi_f(x) = x + \sum_{g,g \neq f} \phi_{f,g}(\lfloor \frac{x}{l^{min}_f} \rfloor)l^{max}_g$
\end{center}
This is the best strict service curve which is tight. 
\end{theorem}

\begin{corollary}
$\beta_f$, the best service curve for flow $f$, can be lower bounded to achieve another three simpler service curves. The first one, $\beta_f'(t)$, is:
\begin{equation}
	\beta_f'(t) =  (\lambda_1 \otimes \nu_{Q_f,q_f + Q_f})  \left(\beta(t) - Q_f\right)
\end{equation}	
Note that $\beta_f'(t)$ is the best strict service for the WRR, it means interleaved WRR offers a better service to a flow of interest in camparision with WRR.\\
Besides, among all rate-latency service curves, one with the minumum latency and one with the maximum rate which are dominant are found. The first one is:
\begin{equation}
	\beta_f''(t) =  B\left( \beta(t) \right)
\end{equation}	
Where $$B: x \mapsto  \beta_{\min\left( \frac{l^{min}_f}{\left( \psi_f(l^{min}_f) - \psi_f(0)    \right)}, \frac{q_f}{q_f + Q_f} \right) , \psi_f(0)}(x)$$ is a rate-latency service curve with the minimum latency. \\
The other one is:
\begin{equation}
	\beta_f'''(t) =  B'\left( \beta(t) \right)
\end{equation}	
Where $$B': x \mapsto \beta_{\frac{q_f}{q_f + Q_f} , Q_f}(x)$$ is a rate-latency service curve with the maximum rate.\\





\end{corollary}

The second strict residual service curve is:
\begin{equation}
	\beta_f'(t) =  B\left( \beta(t) \right)
\end{equation}	
Where $$B: x \mapsto  \beta_{\min\left( \frac{l^{min}_f}{\left( \psi_f(l^{min}_f) - \psi_f(0)    \right)}, \frac{q_f}{q_f + Q_f} \right) , \psi_f(0)}(x)$$ is a rate-latency service curve with the minimum latency that is tight.\\
The third strict residual service curve is:
\begin{equation}
	\beta_f''(t) =  (\lambda_1 \otimes \nu_{Q_f,q_f + Q_f})  \left(\beta(t) - Q_f\right)
\end{equation}	
The fourth strict residual service curve is:
\begin{equation}
	\beta_f'''(t) =  B'\left( \beta(t) \right)
\end{equation}	
Where $$B': x \mapsto \beta_{\frac{q_f}{q_f + Q_f} , Q_f}(x)$$ is a rate-latency service curve with the maximum rate.\\

%%%%%%%% Illustration %%%%%%%
\subsection{Illustration of Strict Service Curves}
To illustrate and compare all strict service curves, the following example is given.
\begin{example}
Let $S$ be a server, offering a strict service of super-additive curve $\beta$, shared by $4$ flows $R_1,...,R_4$, with minimum packet sizes $\{13,15,16,21\}$, maximum packet sizes $\{31,36,32,37\}$, and weights $\{1,4,5,6\}$. Their $\beta_f$, $\beta_f'$, $\beta_f''$, and $\beta_f'''$ are plotted in figure 1.
\begin{figure*}
 \scalebox{1}{\input{test.tex}}
\caption{Strict service curves for each flow of example 1 are plotted. For flow 1, $\beta_f$ and $\beta_f'$ are equal to $\beta_f''$ and $\beta_f'''$ respectively. For others, $\beta_f$ is the most complicated one which offers the best service as well. $\beta_f'$, the best strict service curve of the WRR, is smaller than than $\beta_f$, the best strict service curve of the interleaved WRR. Two rate-latency service curves $\beta_f''$ and $\beta_f'''$, with the minimum latency and the maximum rate respectively, are dominant to any other rate-latency service curves.}
\end{figure*}
\end{example}
%%%%%%%%%%%% Proof %%%%%%%%
\section{Proofs}
The idea of proof is that  we consider a backlogged period $[s,t[$ of flow of interest, $f$. Let $p$ be the number of packets of flow $f$ that are entirely served during this period. Besides, let $C$ be the cycle number when the server serves the first packet of flow $f$ after $s$. Then, for every other flow $g$, the number of packets that are entirely served is upper bounded given $p$ and $C$ (equation \ref{eqn:Numg}). Also, $p$ is upper bounded regarding the amount of service of flow $f$(equation \ref{eqn:Min2}). Combining these two equations gives an implicit inequality for the amount of total service (equation \ref{eqn:TotService}). Inverting the right-hand side of this equation, using the technique of pseudo-inverse, gives a lower bound for amount of service to flow of interest, $f$ (equation \ref{eqn:lsi}). Finally, simplification of the right-hand side of equation \ref{eqn:TotService} gives lower bounds to $\beta_f$, resulting in equations 2,3, and 4.

\subsection{Interleaved WRR Description}
%% %%%%%%%%%%%%Trace Definition of Interleavd WRR%%%%%%%%%%%% 
\begin{definition}[Key Variables]
 Let $[s,t[$ be a backlog period of flow $f$. Let $(\tau_k,fl_k)$ be couples of (instant,flow), printed at line 7 of the algorithm. At line 10 of the algorithm, the server only examines whether a queue is empty or not, however, at line 7, it is already checked that it is not empty and it is the start of a service for that queue. Note that the $\tau_k$ sequence is increasing $(\tau_k<\tau_{k+1})$, since the \texttt{send} instruction has a non-null duration. Let $\tau_{\sigma(0)}$ be the first service opportunity for flow $f$ after $s$ (there is at least one since $s$ marks a backlogged period of $f$), $P$ be the set of complete service opportunities of $f$ between $s$ and $t$, and $p$ its cardinality (if there is no service opportunity between $s$ and $t$, $ P = \emptyset $ and $p = 0$).
	\begin{center}
		$\sigma(0)= \min \{ m | \tau_m \geq s , fl_m = f\}$\\
		$\sigma(k)= \min\{ m | \tau_m > \tau_{\sigma(k-1)},fl_m = f\}$\\
		$P = \{ \tau_m  | s \leq \tau_m, \tau_{m+1} \leq t , fl_m = f \}$\\
		$p = |P|$\\
		%$\sigma(n)= \tau_{m_n}$ such that $n = | \{ \tau_m |\sigma(0) < m \leq m_n, fl_m = f\} |$
	\end{center}
The next service for flow $f$, which will start at $\tau_{\sigma(p)}$, should finish after t. It means it can start either after or before $t$. The following figure shows both cases.
\begin{figure}[h!]
\begin{subfigure}{.5\textwidth}
  \centering
\begin{tikzpicture}
\begin{axis}[%
axis x line=center,
axis y line=none,
xmin=-3,xmax=3,ymin=0, ymax=1,
xtick={-2,2,1.5},
xticklabels={$s$,$\tau_{\sigma(p)}$,$t$}
]
\end{axis}
\end{tikzpicture}
\caption{Next service opportunity starts after $t$.}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
\begin{tikzpicture}
\begin{axis}[%
axis x line=center,
axis y line=none,
xmin=-3,xmax=3,ymin=0, ymax=1,
xtick={-2,1.1,1.5 , 2.2},
xticklabels={$s$,$\tau_{\sigma(p)}$,$t$, $\tau_{\sigma(p) + 1}$}
]
\draw [dotted, <->] (axis cs:1.1,0.05) -- (axis cs:2.2,0.05);
\end{axis}

\end{tikzpicture}
\caption{Next service opportunity starts before $t$.}
\end{subfigure}
\caption{possible backlogged period with $p$ complete services.}
\end{figure}\\
In each service of flow $f$, it will send one packet with at least length of $l^{min}_f$.
	\begin{equation}
		\forall k \geq 0 : R_f^*(\tau_{\sigma(k + 1)}) - R_f^*(\tau_{\sigma(k)}) \geq l^{min}_f
	\end{equation}
Besides, Output of flow $f$ with $p$ complete services in $\left [\tau_{\sigma(0)},\tau_{\sigma(p)} \right[$ is:
	\begin{equation}\label{eqn:Min}
		R_f^*(\tau_{\sigma(p)}) - R_f^*(\tau_{\sigma(0)}) \geq pl^{min}_f
	\end{equation}

\end{definition}

\begin{lemma}
Let $q_{g,f} : [1 , w_f] \mapsto \mathbb{N}$ be the number of visits for some flow $g$ between two consecutive visits of flow $f$ where the second visit occurs at cycle $C_f$ is the following:
	\begin{equation}
		\forall g \neq f: q_{g,f}(C_f) = \begin{cases}1 < C_f \leq w_f \Longrightarrow \begin{cases}
																		0	& w_g < C_f\\
																		1	& w_g \geq C_f\\
																\end{cases}\\
										C_f = 1 \Longrightarrow \left[w_g - w_f\right]^+ + 1
									\end{cases}
	\end{equation}
\end{lemma}
\begin{proof}
According to the algorithm, flow $f$ is visited only in the first $w_f$ cycles of each round. Let consider two cases. The first case is that both visits occur in one round. The second case is that the second visit occurs in the next round. Since $C_f$ is the cycle that is printed at line 6 of the algorithm for the second visit of flow $f$, These two cases can be written as below.\\
\textbf{Case 1:} $1 < C_f \leq w_f$:\\
In this case, the first visit happens in the same round since queue $f$ was visited in cycle $C_f - 1$. Therefore, queues that are after queue $f$ in cycle $C_f - 1$ were visited in the rest of the cycle, and queues that are before queue $f$ in cycle $C_f$ were also visited. Hence, only queues with either $w_g \geq w_f$ or $w_g \geq C_f $ were visited once, and since in this case $C_f  \leq w_f$:
	\begin{equation*}
		1 < C_f \leq w_f \Longrightarrow \forall g \neq f: q_{g,f}(C_f) = \begin{cases}
										0	& w_g < C_f \\
										1	& w_g \geq C_f \\
									\end{cases}
	\end{equation*}
\textbf{Case 2:} $C_f  = 1$\\
In this case, the first visit was in the last cycle of a round that includes $f$. Hence, queues that are after queue $f$ in cycle $w_f$ of the last round were visited in the rest of the cycle, queues with larger weight were visited on the rest of the cycles of that round, and queues with smaller weights were visited at the first cycle of the next round. Therefore, queues with weights larger than $w_f$ were visited once in the rest of the cycle $w_f$, and besides, they were visited during next $(w_g - w_f)$ cycles as well. Queues with smaller weight were visited once at the first cycle of the next round. Thereby:
	\begin{equation*}
		C_f = 1 \Longrightarrow \forall g \neq f: q_{g,f}(C_f) = \begin{cases}
										w_g - w_f + 1	& w_g > w_f\\
										1	& w_g \geq w_f \\
									\end{cases}
	\end{equation*}
Which can be rewitten:
	\begin{equation*}
		C_f = 1 \Longrightarrow \forall g \neq f: q_{g,f}(C_f)=   \left[w_g - w_f\right]^+ + 1
	\end{equation*}
\end{proof}

\begin{lemma}
For any backlogged period $[s,t[$ of flow $f$ such that there are $p$ complete services of flow $f$ and the first service starts at cycle number $C$ (cycle number at time $\tau_{\sigma(0)}$), the number of visits to flow $g \neq f$ is at most $q'_{g,f}\left(C , p \right)$ in $[s , \tau_{\sigma(p)}[$.
	\begin{equation}
		\begin{aligned}
		&\forall g \neq f : q'_{g,f}\left(C, p \right) = \\
		&\sum_{k=0}^{p} q_{g,f} \left( \left (\left( C + k - 1\right) \mod w_f \right)+ 1 \right)
		\end{aligned}
	\end{equation}
Besides, let $C'$ be the cycle number at $\tau_{\sigma(p)}$. Then:
	\begin{equation}
		C' =  \left( C + p - 1\right) \mod w_f + 1 
	\end{equation}
\end{lemma}
\begin{proof}
It can be proved by induction on $p$. \\
\textbf{Base Case:} $ p = 0$\\
In this case, $q'_{g,f}\left(C , 0 \right)$ is the number of visits of flow $g$ between two consecutive visits of flow $f$, which is what we have computed in lemma 1. Therefore:\\
	\begin{equation}
		p = 0 \Longrightarrow \forall g \neq f : q'_{g,f}\left(C , 0 \right) = q_{g,f}(C) 
	\end{equation}
Also, if $p = 0$ then $C = C'$ since $ \left( C - 1\right) \mod w_f + 1  = C$. \\
\textbf{Assume for p - 1 holds}:\\
In this case, we assume that equations 8 and 9 hold for $p - 1$, and we want to show that they also hold for $ p $. First, let prove equation 9. Let $C'$ be the cycle number at $\tau_{\sigma(p - 1)}$, and $C''$ be the cycle number at $\tau_{\sigma(p )}$. Note that:
\begin{equation*}
	(x + 1) \mod w  = \begin{cases} (x \mod w) + 1 	&0 \leq (x \mod w) < w - 1\\
							0			& Otherwise.
				\end{cases}
\end{equation*}
Also, we know that $C'= \left( C + (p-1) - 1\right) \mod w_f + 1$. There will be two cases. If $C' = w_f$, then $C'' = 1$ and moreover, $\left( C + (p-1) - 1\right) \mod w_f + 1 = w_f$ which means $\left( C + (p-1) - 1\right) \mod w_f =w_f - 1$.  By applying this, in this case, we have $\left( C + p - 1\right) \mod w_f + 1 = 1$ which is proven. For the other case, by applying the short lemma, we have $C'' = C' + 1$. To prove the equation 8, the number of visits for some flow $g$ in $[s , \tau_{\sigma(p)}[$, $N$, can be represents by the number of visits in $[s , \tau_{\sigma(p)}[$, $N_1$, plus the number of visits in $[\tau_{\sigma(p - 1)} , \tau_{\sigma(p)}[$, $N_2$. The following figure demonstrates this.
\begin{figure}[h!]
  \centering
\begin{tikzpicture}
\begin{axis}[%
axis x line=center,
axis y line=none,
xmin=-3,xmax=3,ymin=-2, ymax=1,
xtick={-2,2,1.5, 0.8},
xticklabels={$s$,$\tau_{\sigma(p)}$,$t$,$\tau_{\sigma(p - 1)}$}
]
\draw [dotted, <->] (axis cs:-2,0.05) -- (axis cs:0.8,0.05)  node[pos=0.5, above] {$N1$};
\draw [dotted, <->] (axis cs:0.8,0.05) -- (axis cs:2,0.05)  node[pos=0.5, above] {$N2$};
\draw [dotted, <->] (axis cs:-2,0.5) -- (axis cs:2,0.5)  node[pos=0.5, above] {$N$};
\end{axis}
\end{tikzpicture}
\caption{$N = N_1 + N_2$}
\end{figure}\\
Since $N_1 \leq q'_{g,f}\left(C , p - 1 \right)$ and $N_2 \leq q_{g,f}(C'') $, it can be rewritten as below:
	\begin{equation*}
		N \leq q'_{g,f}\left(C , p - 1 \right) + q_{g,f}(C'')
	\end{equation*}
Therefore, by applying the definition of $ q'_{g,f}$ and $C''$:
	\begin{equation*}	
		\begin{aligned}
		N \leq & \sum_{k=0}^{p - 1} q_{g,f} \left( \left (\left( C + k - 1\right) \mod w_f \right)+ 1 \right) \\
		& + q_{g,f}\left(\left( C + p - 1\right) \mod w_f + 1 \right)
		\end{aligned}
	\end{equation*}
Where the righ-hand side is equal to $ q'_{g,f}(C,p)$. Thereby, It is proven.
\end{proof}

\begin{lemma}\label{lem:numg}
$q'_{g,f}$ can be upper bounded as below:
	\begin{equation}\label{eqn:Numg}
	q'_{g,f}\left(C , p \right) \leq \phi_{f,g}(p)
	\end{equation}
where $$\phi: x \mapsto  \left \lfloor \frac{x}{w_f} \right \rfloor w_g +  \left[w_g - w_f\right]^+ + \min \left( \left(x \mod w_f \right) + 1 , w_g  \right)$$.
\end{lemma}
\begin{proof}
There are several steps that should be proved first.\\
\textbf{1)} $q_{g,f}$ is a wide-sense decreasing function.\\
It is sufficient to show that for any integer $k \in [0 , w_f[$, $q_{g,f}(k + 1) \leq q_{g,f}(k)$. if $k = 1$ it is obvious since it is larger or at least equal to 1 and others are at most one. Otherwise, there will be two cases. If $k \leq w_g < k + 1$, then $q_{g,f}(k + 1) = 0$ and $q_{g,f}(k) = 1$. Otherwise, they will be equal. Thereby, in both cases the property holds.\\
\textbf{2)} For any integer $C \in [1 , w_f]$:
\begin{equation}
\sum_{k=0}^{w_f - 1} q_{g,f} \left( \left (\left( C + k - 1\right) \mod w_f \right)+ 1 \right) = w_g (*)
\end{equation}
Since this is sum of all elements of the set $\{q_{f,g}(k) \}_{k \in [1 , w_f]}$, it can be rewritten as below:
	\begin{equation}
		\sum_{k=0}^{w_f - 1} q_{g,f} \left( \left (\left( C + k - 1\right) \mod w_f \right)+ 1 \right)  = \sum_{k=0}^{w_f - 1} q_{g,f} \left(k + 1 \right)
	\end{equation}
Besides, $q_{g,f}(1) =  \left[w_g - w_f\right]^+ + 1$, and other ones are one if $w_g \geq k+1$ which means the rest of the sum is equal to $\min(w_f - 1, w_g - 1)$. Therefore, the right-hand side which is the total sum is $w_g$.\\
\textbf{3)} For any integer $C \in [1 , w_f]$ and $p \geq 0$:
\begin{equation}
	\begin{aligned}
		q'_{g,f}\left(C , p \right) &=  \left \lfloor \frac{p}{w_f} \right \rfloor w_g \\
						&+ \sum_{k=0}^{p \mod w_f} q_{g,f} \left( \left (\left( C + k - 1\right) \mod w_f \right)+ 1 \right)
	\end{aligned}
\end{equation}
We can write $ p = \left \lfloor \frac{p}{w_f} \right \rfloor w_f + p \mod w_f$. Then, there will $\left \lfloor \frac{p}{w_f} \right \rfloor$ of $(*)$, which is equal to $w_g$, and a sum with the remider part.\\
\textbf{4)} For any integer $p \geq 0$:
\begin{equation}
	\begin{aligned}
			q'_{g,f}\left(1 , p \right) &=  \left \lfloor \frac{p}{w_f} \right \rfloor w_g\\
								&\underbrace{ +  \left[w_g - w_f\right]^+ + \min \left( \left(p \mod w_f \right) + 1 , w_g  \right)}_{\phi_{f,g}(p)}
	\end{aligned}
\end{equation}
By applying the second property, the definition of $q_{g,f}(1)$, and function $\phi_{f,g}$ it is proven.
\textbf{5)} For any integer $C \in [1 , w_f]$ and $p \geq 0$:
\begin{equation}
	\begin{aligned}
			q'_{g,f}\left(C , p \right) \leq  \underbrace{q'_{g,f}\left(1 , p \right)}_{\phi_{f,g}(p)}
	\end{aligned}
\end{equation}
Since, both side is sum of $p \mod w_f + 1$ unique elements of the set $\{q_{f,g}(k) \}_{k \in [1 , w_f]}$ and moreover, by applying the first property, the right hand side is the maximum sum of $p \mod w_f + 1$ unique elements of this set, it is proven. \\

\end{proof}


%% %%%%%%%%%%%%lower bound on the output flow during the backlog of Interleavd WRR%%%%%%%%%%%% 

\subsection{Amount of Service to Flow of Interest}

\begin{Proposition}\label{prop:p}
The number of complete services, $p$, of flow of interest, $f$, in $[s,t[$ can be upper bounded:

Besides, $p$ can be upper bounded:
	\begin{equation}\label{eqn:p}
		p \leq \left \lfloor \frac{R_f^*(t) - R_f^*(s)}{l^{min}_f} \right \rfloor
	\end{equation}
\end{Proposition}

\begin{proof}[\textbf{Proof of Proposition \ref{prop:p}}]
Given equation \ref{eqn:Min}, we claim the following:
	\begin{equation}\label{eqn:Min2}
		R_f^*(t) - R_f^*(s) \geq pl^{min}_f
	\end{equation}
First, since $s \leq \tau_{\sigma(0)}$ and the output flow is a non-decreasing function, $R_f^*(s) \leq R_f^*(\tau_{\sigma(0)})$. It can be claimed that $R_f^*(t) \geq R_f^*(\tau_{\sigma(p)})$. If $t \geq \tau_{\sigma(p)}$, since $R_f^*$ is a wide-sense increasing function, this property holds. Also, if $t < \tau_{\sigma(p)}$, then $t$ is not an instant of the service opportunity of flow $f$ which leads to $R_f^*(t) =R_f^*(\tau_{\sigma(p)})$. In both cases, the property holds. Then, using equation \ref{eqn:Min2}, it is proven.
\end{proof}

\begin{lemma} \label{lem:g}
For every flow $g \neq f$, the following property holds:
	\begin{equation}
		\forall g \neq f: R_g^*(t)  \leq R_g^*(\tau_{\sigma(p)}) 
	\end{equation}
\end{lemma}

\begin{proof}
There will be two cases. If $t \leq \tau_{\sigma(p)}$, since this is a wide-sense increasing function, this property holds. Also, if $t > \tau_{\sigma(p)}$, $t$ is an instant of the service opportunity of flow $f$ which leads to that for all other flows $R_g^*(t) =R_g^*(\tau_{\sigma(p)})$.
\end{proof}



\subsection{Total Amount of  Service}
\begin{lemma} \label{lem:TotService}
Total amount of service can be bounded as a function of service of flow of interest in its backlogged period:
	\begin{equation}\label{eqn:TotService}
		\beta(t-s) \leq \psi_f \left( R_f^*(t) - R_f^*(s) \right)
	\end{equation}
Where $\psi_f$ is defined in definition 3.
\end{lemma}
\begin{proof}
Since the interval $\left[s,t\right[$ is a backlog period, by the definition of the strict sevice curve:
	\begin{equation}
		\beta(t-s) \leq \sum_{k=1}^{n} R_k^*(t) - R_k^*(s) \\
	\end{equation}
	\begin{equation}
		 \Longrightarrow \beta(t-s) \leq (R_f^*(t) - R_f^*(s)) + \sum_{g \neq f} R_g^*(t) - R_g^*(s)
	\end{equation}
Applying lemma \ref{lem:g}:
	\begin{equation}
		\beta(t-s) \leq (R_f^*(t) - R_f^*(s)) + \sum_{g \neq f} R_g^*(\tau_{\sigma(p)}) - R_g^*(s)
	\end{equation}
By applying lemma \ref{lem:numg}, each flow $g$ is visited at most $\phi_{f,g}(p)$ during the interval $\left[s,\tau_{\sigma(p)}\right[$. Thereby:
	\begin{equation}
		\beta(t-s) \leq (R_f^*(t) - R_f^*(s)) + \sum_{g \neq f} \phi_{f,g}(p)l^{max}_g 
	\end{equation}
By applying proposition \ref{prop:p}:
	\begin{equation}
		\begin{aligned}
		\beta(t-s) & \leq (R_f^*(t) - R_f^*(s)) \\
				&\underbrace{+\sum_{g,g \neq f} \phi_{f,g}\left( \left \lfloor \frac{R_f^*(t) - R_f^*(s)}{l^{min}_f } \right \rfloor \right)l^{max}_g }_{\psi_f(R_f^*(t) - R_f^*(s))}
		\end{aligned}
	\end{equation}
Where $\psi_f$ is defined in definition 3:
	\begin{equation}
		\beta(t-s) \leq \psi_f \left(R_f^*(t) - R_f^*(s) \right)
	\end{equation}
\end{proof}

\subsection{Lower Pseudo-inverse Technique}
\subsubsection{Definition of Lower Pseudo-inverse}
\begin{definition}
Let $f : x \mapsto f(x)$ be a non-decreasing function. The lower pseudo-inverse function $f^{\downarrow}$ is given by:
\begin{equation}
f^{\downarrow}(y) = \inf \{x | f(x) \geq y \} = \sup \{ x | f(x) < y \}
\end{equation}
\end{definition}

\subsubsection{Properties of Lower Pseudo-inverse}
The following lemma is an important part of the proofs.
\begin{lemma} \label{lem:lsi}
Let $\psi : x \mapsto \psi(x)$ be a wide-sense increasing function. Also, let $\psi^{\downarrow}$ be its lower pseudo-inverse. Then:
\begin{equation}
y \leq \psi(x) \Longrightarrow x \geq \psi^{\downarrow}(y)
\end{equation}
\end{lemma}
We need to find the lower-pseudo inverse of $\psi(x)$ to bound the amount of service of flow of interest. To do so, first, we should show that $\psi(x)$ is a wide-sense increasing function.
\begin{Proposition} \label{prop:wsi}
$\psi(x)$ is a wide-sense increasing function.
\end{Proposition}

\begin{proof}[\textbf{Proof of Proposition \ref{prop:wsi}}]
It is sufficient to show that $\phi_{f,g}$ is a wide-sense increasing function. For any non-negative integers $x$ and $y$ such that $y \leq x$. One can write $x = kw_f + (x \mod w_f)$ and $y = k'w_f+ (y \mod w_f)$ where $k,k'$ are non-negative integers. There will be two cases:\\
\textbf{case1:} $k=k'$\\
In this case, we know that $(y \mod w_f \leq x \mod w_f)$ and $(\left \lfloor \frac{x}{w_f} \right \rfloor =\left \lfloor \frac{y}{w_f} \right \rfloor)$. Therefore, $ \phi_{f,g}(y) \leq \phi_{f,g}(x)$.\\
\textbf{case2:} $k > k'$\\
In this case, $(\left \lfloor \frac{x}{w_f} \right \rfloor > \left \lfloor \frac{y}{w_f} \right \rfloor)$. Thereby, $\phi_{f,g}(x)$ is at least one $w_g$ larger. Hence, $ \phi_{f,g}(y) \leq \phi_{f,g}(x)$.
\end{proof}

Given equation \ref{eqn:TotService} and proposition \ref{prop:wsi}, by applying lemma \ref{lem:lsi}, the following equation is driven:
	\begin{equation} \label{eqn:fService}
		(R_f^*(t) - R_f^*(s)) \geq \psi_f^{\downarrow}(\beta(t-s))  
	\end{equation}





%%%%%%% Function Definition%%%%
\subsection{Close form for the Right-hand Side of Equation \ref{eqn:fService}}
First, let consider the following proposition.
\begin{Proposition} \label{prop:lsi}
Let $f: x \mapsto x + a \left( 1 + \left \lfloor \frac{x}{b} \right \rfloor \right)$ which is a wide-sense increasing function. Then, $f$ has a lower pseudo-inverse $f^{\downarrow}(y) = \lambda_1 \otimes \nu_{b,a+b}(y - a)$.
\begin{figure}[H]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
\begin{tikzpicture}


	\pgfplotsset{soldot/.style={color=black,only marks,mark=*}} 				   		   		 \pgfplotsset{holdot/.style={color=black,fill=white,only marks,mark=*}}
	\pgfplotsset{ticks=none}
	\begin{axis}[xlabel=$x$, ylabel=$x + a \lfloor \frac{x}{b} \rfloor + c$,
	xmin=-2,xmax= 8,ymin=-2,ymax=8, axis lines=center, width=0.75\textwidth,
       height=0.55\textwidth,]

	\addplot[soldot] coordinates{(0,1)(1,3)(2,5) };
	\addplot[holdot] coordinates{(1,2)(2,4) (3,6)} ;

	\draw[dashed] (axis cs:0,0) -- (axis cs:0,1);
	\draw[ultra thick] (axis cs:0,1) -- (axis cs:1,2);
	\draw[dotted] (axis cs:1,0) -- (axis cs:1,2);
	\draw[dotted] (axis cs:0,2) -- (axis cs:1,2);

	\draw[dashed] (axis cs:1,2) -- (axis cs:1,3);
	\draw[ultra thick] (axis cs:1,3) -- (axis cs:2,4);
	\draw[dotted] (axis cs:2,0) -- (axis cs:2,4);


%% W1
	\draw[dashed] (axis cs:2,4) -- (axis cs:2,5);
	\draw[ultra thick] (axis cs:2,5) -- (axis cs:3,6);
	\draw[dotted] (axis cs:3,0) -- (axis cs:3,6);

%%
	\draw[dotted] (axis cs:3,6.5) -- (axis cs:4,7.5);


%x axis
\draw (1,-1) node{$b$};
\draw (2,-1) node{$2b$};
\draw (3,-1) node{$3b$};
\draw (4,-1) node{$4b$};
\draw (5,-1) node{...};

%y axis
\draw (-1,1) node{$a$};
\draw (-1,2) node{$a + b$};
\draw (-1,4) node{.};
\draw (-1,5) node{.};
\draw (-1,6) node{.};

%%a part

	\draw[dotted, <->] (axis cs:1.2,2) -- (axis cs:1.2,3) node[pos=0.5, right] {$a$};
	\draw[dotted, <->] (axis cs:2.2,4) -- (axis cs:2.2,5) node[pos=0.5, right] {$a$};
	\end{axis}
\end{tikzpicture}% NO EMPTY LINE HERE!!!! 
\caption{$f(x)$}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
\begin{tikzpicture}


	\pgfplotsset{soldot/.style={color=black,only marks,mark=*}} 				   		   \pgfplotsset{holdot/.style={color=black,fill=white,only marks,mark=*}}
	\pgfplotsset{ticks=none}
	\begin{axis}[xlabel=$y$, ylabel=$f^{-1}(y)$,
	xmin=-2,xmax=8,ymin=-2,ymax=8, axis lines=center, width=0.75\textwidth,
       height=0.55\textwidth,]

	\draw[ultra thick] (axis cs:0,0) -- (axis cs:1,0);
	\draw[ultra thick] (axis cs:1,0) -- (axis cs:2,1);
	\draw[dotted] (axis cs:0,1) -- (axis cs:2,1);

	\draw[ultra thick] (axis cs:2,1) -- (axis cs:3,1);
	\draw[ultra thick] (axis cs:3,1) -- (axis cs:4,2);
	\draw[dotted] (axis cs:0,2) -- (axis cs:4,2);
	\draw[dotted] (axis cs:3,0) -- (axis cs:3,1);

%% W1
	\draw[ultra thick] (axis cs:4,2) -- (axis cs:5,2);
	\draw[ultra thick] (axis cs:5,2) -- (axis cs:6,3);
	\draw[dotted] (axis cs:0,3) -- (axis cs:6,3);
	\draw[dotted] (axis cs:3,0) -- (axis cs:3,1);

%%
	\draw[dotted] (axis cs:6.5,3) -- (axis cs:7.5,4);


%x axis
\draw (3,-1) node{$2a + b$};
\draw (6,-1) node{...};

%y axis
\draw (-1,1) node{$b$};
\draw (-1,2) node{$2b$};
\draw (-1,3) node{$3b$};
\draw (-1,4) node{.};
\draw (-1,5) node{.};
\draw (-1,6) node{.};

%%a part

	\draw[dotted, <->] (axis cs:0,0.2) -- (axis cs:1,0.2) node[pos=0.5, above] {$a$};
	\draw[dotted, <->] (axis cs:2,1.2) -- (axis cs:3,1.2) node[pos=0.5, above] {$a$};
	\draw[dotted, <->] (axis cs:4,2.2) -- (axis cs:5,2.2) node[pos=0.5, above] {$a$};
	\end{axis}
\end{tikzpicture} 
\caption{$f^{-1}(y)$}
\end{subfigure}
\caption{Function $f$ and its lower-pseudo inverse} 
\end{figure}  
\end{Proposition}
For a better illustration, function $\psi_f$ is plotted below:
\begin{figure}[H]
\centering
\begin{tikzpicture}

	\pgfplotsset{soldot/.style={color=black,only marks,mark=*}} 				   		   \pgfplotsset{holdot/.style={color=black,fill=white,only marks,mark=*}}
	\pgfplotsset{ticks=none}
	\begin{axis}[xlabel=$x$, ylabel=$\psi_f(x)$,
	xmin=0,xmax=15,ymin=-2,ymax=25, axis lines=center, width=0.5\textwidth,
       height=0.5\textwidth,]

	\addplot[soldot] coordinates{(0,2.4)(1,4.4)(2,6.2) (3,8) (7,13)  (8,14.5) (9,16) (10,19.4) (11,21.4) };
	\addplot[holdot] coordinates{(1,3.3)(2,5.4) (3,7.2) (4,9) (7,12.5) (8,14)  (9,15.5) (10,17) (11,20.4) (12,22.4)  } ;

	\draw[dashed] (axis cs:0,0) -- (axis cs:0,2.4);
	\draw[ultra thick] (axis cs:0,2.4) -- (axis cs:1,3.4);

	\draw[dashed] (axis cs:1,3.4) -- (axis cs:1,4.4);
	\draw[ultra thick] (axis cs:1,4.4) -- (axis cs:2,5.4);

%% W1
	\draw[dashed] (axis cs:2,5.4) -- (axis cs:2,6.2);
	\draw[ultra thick] (axis cs:2,6.2) -- (axis cs:3,7.2);

	\draw[dashed] (axis cs:3,7.2) -- (axis cs:3,8);
	\draw[ultra thick] (axis cs:3,8) -- (axis cs:4,9);


%%
	\draw[dotted] (axis cs:5,10.4) -- (axis cs:6,11.4);


%%W2
	\draw[dashed] (axis cs:7,12.5) -- (axis cs:7,13);
	\draw[ultra thick] (axis cs:7,13) -- (axis cs:8,14);

	\draw[dashed] (axis cs:8,14) -- (axis cs:8,14.5);
	\draw[ultra thick] (axis cs:8,14.5) -- (axis cs:9,15.5);

	\draw[dashed] (axis cs:9,15.5) -- (axis cs:9,16);
	\draw[ultra thick] (axis cs:9,16) -- (axis cs:10,17);

%% W_i 
%%% Second set
	\draw[dashed] (axis cs:10,17) -- (axis cs:10,19.4);
	\draw[ultra thick] (axis cs:10,19.4) -- (axis cs:11,20.4);

	\draw[dashed] (axis cs:11,20.4) -- (axis cs:11,21.4) ;
	\draw[ultra thick] (axis cs:11,21.4) -- (axis cs:12,22.4);

%%
	\draw[dotted] (axis cs:13,23.4) -- (axis cs:14,24.4);



	\draw[dotted, <->] (axis cs:0.2,0) -- (axis cs:0.2,2.4) node[pos=0.5, right] {$L_f$};
%	\draw[dotted, <->] (axis cs:1.2,2) -- (axis cs:1.2,3) node[pos=0.5, right] {$(n-1)l$};
%	\draw[dotted, <->] (axis cs:2.2,4) -- (axis cs:2.2,4.8) node[pos=0.5, right] {$(n-2)l$};
%	\draw[dotted, <->] (axis cs:3.2,5.8) -- (axis cs:3.2,6.6) node[pos=0.5, right] {$(n-2)l$};
%\draw[dotted, <->] (axis cs:7.2,11.1) -- (axis cs:7.2,11.6) node[pos=0.5, right] {$(n-i)l$};
%	\draw[dotted, <->] (axis cs:8.2,12.6) -- (axis cs:8.2,13.1) node[pos=0.5, right] {$(n-i)l$};
%	\draw[dotted, <->] (axis cs:9.2,14.1) -- (axis cs:9.2,14.6) node[pos=0.5, right] {$(n-i)l$};
%	\draw[dotted, <->] (axis cs:9.2,14.1) -- (axis cs:9.2,14.6) node[pos=0.5, right] {$(n-i)l$};
	\draw[dotted, <->] (axis cs:10.2,17) -- (axis cs:10.2,19.4) node[pos=0.5, right] {$L_f$};
	\draw[dotted, <->] (axis cs:0,3.4) -- (axis cs:1,3.4) node[pos=0.65, above] {$l^{min}_f$};
%	\draw[dotted, <->] (axis cs:11.2,19) -- (axis cs:11.2,20) node[pos=0.5, right] {$(n-1)l$};

%	\draw[dotted] (axis cs:7,12.5) -- (axis cs:7,0);
	\draw[dotted] (axis cs:10,17) -- (axis cs:10,0);

%% x axis
%\draw (1,-1) node{$l^{min}_f$};
%\draw (2,-1) node{$w_1l$};
%\draw (3,-1) node{$3l$};
%\draw (4,-1) node{$4l$};
%\draw (5.5,-1) node{...};
%\draw (7,-1) node{$w_{f-1}l$};
\draw (10,-1) node{$w_fl$};
%\draw (8.5,-1) node{$....$};




	\end{axis}




\end{tikzpicture}
\caption{$\psi_f(x) = x + \sum_{g,g\neq f} \phi_{f,g}(\lfloor \frac{x}{l^{min}_f} \rfloor)l^{max}_g$}
\end{figure}
By comparing function $f(x)$ in prroposition \ref{prop:lsi} and $\psi_f$, sum of $w_f$ shifted version of $f$ (with $a = l^{min}_f$ and $b = L_{tot}$), where they are shifted regrading $\psi_f(kl^{min}_f)$ with $k \in [0 \, w_f[$, by applying proposition \ref{prop:lsi}:
\begin{equation} \label{eqn:lsi}
\psi_f^{\downarrow}(x) =  (\lambda_1 \otimes U_f)(x)
\end{equation}
Where $$U_f(x) =\sum_{k=0}^{w_f - 1}\left( \nu_{l^{min}_f,L_{tot}} \otimes \delta_{\psi_f(kl^{min}_f))} \right) (x)$$ with $L_{tot} = q_f + Q_f$.\\
The lower pseudo-inverse is plotted as well:
\begin{figure}[H]
\begin{tikzpicture}

	\pgfplotsset{soldot/.style={color=black,only marks,mark=*}} 				   		   \pgfplotsset{holdot/.style={color=black,fill=white,only marks,mark=*}}
	\pgfplotsset{ticks=none}
	\begin{axis}[ylabel = $\psi_f^{\downarrow}$,xmin=-3,xmax=28,ymin=-2.1,ymax=13, axis lines=center,width=0.5\textwidth,height=0.5\textwidth]
	\draw[ultra thick] (axis cs:0,0) -- (axis cs:2.4,0) ;
	\draw[ultra thick] (axis cs:2.4,0) -- (axis cs:3.4,1);

	\draw[ultra thick] (axis cs:3.4,1) -- (axis cs:4.4,1);
	\draw[ultra thick] (axis cs:4.4,1) -- (axis cs:5.4,2);

%% W1
	\draw[ultra thick] (axis cs:5.4,2) -- (axis cs:6.2,2);
	\draw[ultra thick] (axis cs:6.2,2) -- (axis cs:7.2,3);

	\draw[ultra thick] (axis cs:7.2,3) -- (axis cs:8,3);
	\draw[ultra thick] (axis cs:8,3) -- (axis cs:9,4);

%%
	\draw[dotted] (axis cs:9.4,5) -- (axis cs:10.4,6);




%%W2
	\draw[ultra thick] (axis cs:12.5,7) -- (axis cs:13,7);
	\draw[ultra thick] (axis cs:13,7) -- (axis cs:14,8);

	\draw[ultra thick] (axis cs:14,8) -- (axis cs:14.5,8);
	\draw[ultra thick] (axis cs:14.5,8) -- (axis cs:15.5,9);

	\draw[ultra thick] (axis cs:15.5,9) -- (axis cs:16,9);
	\draw[ultra thick] (axis cs:16,9) -- (axis cs:17,10);

%% W_i 
%%% Second set
	\draw[ultra thick] (axis cs:17,10) -- (axis cs:19.4,10);
	\draw[ultra thick] (axis cs:19.4,10) -- (axis cs:20.4,11);

	\draw[ultra thick] (axis cs:20.4,11) -- (axis cs:21.4,11) ;
	\draw[ultra thick] (axis cs:21.4,11) -- (axis cs:22.4,12);

%%

%	\draw[dotted] (axis cs:12.5,7) -- (axis cs:0,7);
	\draw[dotted] (axis cs:17,10) -- (axis cs:0,10);
%
	\draw[dotted] (axis cs:0,1) -- (axis cs:3.4,1);
%	\draw[dotted] (axis cs:5.4,2) -- (axis cs:0,2);
%	\draw[dotted] (axis cs:7.2,3) -- (axis cs:0,3);
	\draw[dotted] (axis cs:19.4,10) -- (axis cs:19.4,0);
	\draw[dotted] (axis cs:4.4,1) -- (axis cs:4.4,0);

%% y axis
\draw (-1,1) node{$l^{min}_f$};
%\draw (-1,2) node{$w_1$};
%\draw (-1,3) node{$3$};
%\draw (-1,4) node{.};
%\draw (-1,5) node{.};
%\draw (-1,6) node{.};
%\draw (-1,7) node{$w_{f-1}$};
\draw (-1,10) node{$w_fl^{min}_f$};
%\draw (-1,9) node{$.$};
%\draw (-1,8) node{$.$};
%\draw (-1,8.5) node{$.$};
%% xaxis
%\draw (2,-1) node{$\psi_f(0)$};
\draw (4.4,-1) node{$\psi_f(l^{min}_f)$};
\draw (19.4,-1) node{$\psi_f(w_fl^{min}_f)$};





\end{axis}

\end{tikzpicture}
\caption{Function $\psi_f^{\downarrow}$, lower-pseudo inverse function of $\psi_f$.}
\end{figure}

\subsection{Proof of Equation 1}
\begin{proof}[\textbf{Proof of Equation 1}]
Combining equations \ref{eqn:fService} and \ref{eqn:lsi}:
\begin{equation}
\underbrace{ R_f^*(t) - R_f^*(s) }_{\beta_f \left( t - s\right)} = \left( \lambda_1 \otimes U_f \right) \left( \beta \left( t - s \right) \right)
\end{equation}	
\end{proof}
	

